Two ways to make your robot proactive: reasoning about human intentions, or reasoning about possible futures

Robots sharing their space with humans need to be proactive in order to be helpful. Proactive robots are able to act on their own initiative in an anticipatory way to benefit humans. In this work, we investigate two ways to make robots proactive. One way is to recognize humans' intentions and to act to fulfill them, like opening the door that you are about to cross. The other way is to reason about possible future threats or opportunities and to act to prevent or to foster them, like recommending you to take an umbrella since rain has been forecasted. In this paper, we present approaches to realize these two types of proactive behavior. We then present an integrated system that can generate proactive robot behavior by reasoning on both factors: intentions and predictions. We illustrate our system on a sample use case including a domestic robot and a human. We first run this use case with the two separate proactive systems, intention-based and prediction-based, and then run it with our integrated system. The results show that the integrated system is able to take into account a broader variety of aspects that are needed for proactivity.

==> conclusion.tex <==
%----------------------------------------------------------------------------
\section{Conclusion}\label{sec:con}
%----------------------------------------------------------------------------
In this paper, we \CN{present a method to generate proactive robot behavior.} We \CN{show and discuss a first version of an integration of} to two stand-alone approaches to proactivity: $\eqm $, equilibrium maintenance, that infers opportunities for acting based on reasoning about the robot’s possible actions, prediction about the future development of the state and about what is preferable; and $\uir$, human intention reasoning, that infers what to do next by recognizing the human’s current intention and taking over doing the next action in the human’s plan of acting. We show the benefits of both system that the other system is unable to produce such as; $\uir$ focuses on helping humans towards their intentions, \CN{whereas} $\eqm$ focuses on preventing humans to end up in undesirable situations. \CN{$\eqm$ (as of now) is ignorant of human intentions and therefore cannot generate proactive behavior to support the human to achieve them.} On the other hand, $\uir$ does not reason about \CN{how the state will evolve in the future and what is the overall desirability of different states, hence, it cannot generate proactive behavior based on reasoning on prediction of the state and benefit of acting effects. On a use case we first show the proactive behavior of $\uir$; we then show on the same use case the proactive behavior of $\eqm$; finally we apply a combination of both systems, $\uir$ and $\eqm$, on this very use case and observe the resulting proactive behavior. The use case is implemented and tested in a computer program with terminal input (state evolution) and output (inferred robot action). We show that the novel combined solution of $\uir$ and $\eqm$ achieves the best proactive behavior as it can take into account the intentions of the human, the desirability of state and benefit of action effects as well as prediction of the future state evolution. }  

\SB{In future, we plan to test our system in a real robot system. In the current paper, we demonstrated our results on a imagined domestic robot that is capable of manipulating the world physically, but the implementation has been confined to the computer with inputs and outputs to the screen. We plan to use the Pepper Humanoid robot (which is described in \citep{Pandey2018AKind}) to conduct experiments akin to the ones described in Section~\ref{sec:exp}.  
%The Pepper robot is not capable of physically manipulating the world. Therefore why all actions are defined as communicative actions, and speech executor is added to the system. Physical manipulation adds another layer of challenges such as detection, grasping, etc. By using communicative action, we are also eliminating some of those challenges. On the other hand, any robot and domain could be used by defining actions, executors of the robot, scenario, and possible human goals. 
} 
Apart from Pepper, our system is general enough that should be able to implement it on a great variety of physical robots or simulated agents, in diverse domains. 
%--------------------------------------------------------------------------------
% EOF
%--------------------------------------------------------------------------------

==> intro.tex <==
%----------------------------------------------------------------------------
\section{Introduction}\label{sec:intro}
%----------------------------------------------------------------------------

Robots sharing the same spaces as humans, are preferred to be proactive by humans~\citep{harman2020action, pandey2013towards}. 
However, a major part of the work on AI systems and robots are reactive --- responding to explicit requests and external events. 
Some more recent work on making artificial agents and robots proactive exist, but often the solutions are domain-specific and prescriptive~\citep{umbrico2020holistic,
  sirithunge2019proactive, peng2019design, harman2020action, kc2019case,
  bremner2019proactive}. 
In this work, we aim to address the question of finding a general solution to make robots proactive taking into account the human and their intention.
By proactive we mean the robot is able to act anticipatory and on own initiative. This definition follows the one in organizational psychology~\citep{grant2008the}. Acting on own initiative means the robot generates its own goals and decides which of them to pursue and when. Such a reasoning in particular needs to include prediction how the environment will evolve and what the human intends to and will do. 
In our work we generate and select among opportunities for acting based on prediction of the state and intention of the human, as well as reasoning about what is desirable in general. 
In particular, we propose a framework that is domain-unspecific and declarative and is able to reason on the benefit of acting now or later. Taking into account the knowledge and intention of the human, the framework predicts how the state will evolve and finds opportunities for acting that bring the system into a more desirable state.

The contributions of this paper are as follows: (i)~we introduce a framework that is able to infer acting decisions proactively, that is, on own initiative, based on prediction of how the state will evolve, reasoning about the robot's capabilities and what is overall desirable, and on based on user intention recognition; (ii)~we show how the user intention recognition can reduce the load of the state prediction by being able neglect directions in which the state can evolve based on the user's intention; (iii)~in experimental evaluation we show the benefit of having a system with both user intention recognition and proactivity to achieve the most favorable outcomes.

Contributions:
(i)~Improving Interaction between human and robot; 
Including improving robot’s trustability, transparency and legibility
(ii)~Preventing potential undesired outcomes; which occurs lack of knowledge
(iii)~Knowledge Repair; correcting user belief about world by inferring user’s actions and reality

The remainder of this paper is organized as follows. In Section~\ref{sec:sota} we give an overview of the state-of-the-art in proactive artificial agents and robots, as well as human intention recognition. Section~\ref{sec:sys} describes the theoretical framework used in our system. In Section~\ref{sec:exp} we show the experiments we conducted. We discuss the outcomes of the experiments and some future directions in Section~\ref{sec:disc}, before we conclude in Section~\ref{sec:con}.
Finally, in Section~\ref{sec:con} we conclude.














%--------------------------------------------------------------------------------
% EOF
%--------------------------------------------------------------------------------
